Generalizable Imitation Learning Through Pre-Trained Representations

In this paper, we leverage self-supervised vision transformer models and their emergent semantic abilities to improve the generalization abilities of imitation learning policies. We introduce DVK, an imitation learning algorithm that leverages rich pre-trained Visual Transformer patch-level embeddings to obtain better generalization when learning through demonstrations. Our learner sees the world by clustering appearance features into groups associated with semantic concepts, forming stable keypoints that generalize across a wide range of appearance variations and object types. We demonstrate how this representation enables generalized behaviour by evaluating imitation learning across a diverse dataset of object manipulation tasks. To facilitate further study of generalization in Imitation Learning, all of our code for the method and evaluation, as well as the dataset, is made available.

==> table_graveyard.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Object} &  \multicolumn{9}{c} {Method}\\
\cmidrule{3-11}
& & ViT           & BC$_\text{base}$ & BC$_\text{dino}$ & BC & BC-RNN$_\text{base}$ & BC-RNN$_\text{dino}$ & BC-RNN & R3M$_\text{SM}$ & R3M$_\text{flat}$ \\ \midrule
Train   & (Blue, Flower, Yellow)    & 0.62          & 0.50            & 0.41            & 0.51               & 0.70            & \textbf{0.72}   & 0.45               & 0.28    & 0.49      \\
Test    & White                     & \textbf{0.47} & 0.13            & 0.26            & 0.40               & 0.24            & 0.40            & 0.29               & 0.08    & 0.07      \\ \midrule
Train   & (Blue, White, Yellow)     & 0.62          & 0.48            & 0.48            & 0.48               & \textbf{0.70}   & 0.70            & 0.42               & 0.22    & 0.46      \\
Test    & Flower                    & \textbf{0.29} & 0.12            & 0.17            & 0.23               & 0.22            & \textbf{0.29}   & 0.07               & 0.11    & 0.00      \\ \midrule
Train   & (Flower, White, Yellow)   & 0.62          & 0.48            & 0.46            & 0.54               & 0.72            & \textbf{0.75}   & 0.47               & 0.29    & 0.51      \\
Test    & Blue                      & \textbf{0.44} & 0.01            & 0.09            & 0.14               & 0.07            & 0.32            & 0.15               & 0.00    & 0.00      \\ \midrule
Train   & (Blue, Flower, White)     & 0.57          & 0.43            & 0.43            & 0.44               & \textbf{0.69}   & 0.68            & 0.42               & 0.24    & 0.47      \\
Test    & Yellow                    & \textbf{0.63} & 0.17            & 0.07            & 0.47               & 0.31            & 0.17            & 0.37               & 0.05    & 0.06      \\ \midrule
\multicolumn{2}{l}{In-Distribution Average}   & 0.61          & 0.47            & 0.45            & 0.49               & 0.70            & \textbf{0.71}   & 0.44               & 0.26    & 0.48      \\
\multicolumn{2}{l}{Out-Of-Distribution Average}    & \textbf{0.46} & 0.11            & 0.15            & 0.31               & 0.21            & 0.29            & 0.22               & 0.06    & 0.03      \\ \bottomrule \\
\end{tabular}
\caption{Success rate on }
\end{table*}

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Object} &  \multicolumn{9}{c} {Method}\\
\cmidrule{3-11}
& & ViT           & BC$_\text{base}$ & BC$_\text{dino}$ & BC & BC-RNN$_\text{base}$ & BC-RNN$_\text{dino}$ & BC-RNN & R3M$_\text{SM}$ & R3M$_\text{flat}$ \\ \midrule
Train     & (Blue, Flower, Yellow)  & 0.62 \textcolor{gray}{$\pm$ 0.10}           & 0.50 \textcolor{gray}{$\pm$ 0.10}                     & 0.41 \textcolor{gray}{$\pm$ 0.10}                     & 0.51 \textcolor{gray}{$\pm$ 0.09}                        & 0.70 \textcolor{gray}{$\pm$ 0.10}                     & \textbf{0.72 \textcolor{gray}{$\pm$ 0.06}}            & 0.45 \textcolor{gray}{$\pm$ 0.09}                        & 0.28 \textcolor{gray}{$\pm$ 0.13}              & 0.49 \textcolor{gray}{$\pm$ 0.10}                \\
Test      & White                   & \textbf{0.47 \textcolor{gray}{$\pm$ 0.09}}  & 0.13 \textcolor{gray}{$\pm$ 0.08}                     & 0.26 \textcolor{gray}{$\pm$ 0.06}                     & 0.40 \textcolor{gray}{$\pm$ 0.04}                        & 0.24 \textcolor{gray}{$\pm$ 0.00}                     & 0.40 \textcolor{gray}{$\pm$ 0.05}                     & 0.29 \textcolor{gray}{$\pm$ 0.12}                        & 0.08 \textcolor{gray}{$\pm$ 0.09}              & 0.07 \textcolor{gray}{$\pm$ 0.03}                \\ \midrule
Train     & (Blue, White, Yellow)   & 0.62 \textcolor{gray}{$\pm$ 0.05}           & 0.48 \textcolor{gray}{$\pm$ 0.08}                     & 0.48 \textcolor{gray}{$\pm$ 0.14}                     & 0.48 \textcolor{gray}{$\pm$ 0.12}                        & \textbf{0.70 \textcolor{gray}{$\pm$ 0.10}}            & 0.70 \textcolor{gray}{$\pm$ 0.07}                     & 0.42 \textcolor{gray}{$\pm$ 0.11}                        & 0.22 \textcolor{gray}{$\pm$ 0.08}              & 0.46 \textcolor{gray}{$\pm$ 0.09}                \\
Test      & Flower                  & \textbf{0.29 \textcolor{gray}{$\pm$ 0.05}}  & 0.12 \textcolor{gray}{$\pm$ 0.05}                     & 0.17 \textcolor{gray}{$\pm$ 0.02}                     & 0.23 \textcolor{gray}{$\pm$ 0.05}                        & 0.22 \textcolor{gray}{$\pm$ 0.09}                     & \textbf{0.29 \textcolor{gray}{$\pm$ 0.05}}            & 0.07 \textcolor{gray}{$\pm$ 0.04}                        & 0.11 \textcolor{gray}{$\pm$ 0.01}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\ \midrule
Train     & (Flower, White, Yellow) & 0.62 \textcolor{gray}{$\pm$ 0.08}           & 0.48 \textcolor{gray}{$\pm$ 0.10}                     & 0.46 \textcolor{gray}{$\pm$ 0.10}                     & 0.54 \textcolor{gray}{$\pm$ 0.09}                        & 0.72 \textcolor{gray}{$\pm$ 0.08}                     & \textbf{0.75 \textcolor{gray}{$\pm$ 0.08}}            & 0.47 \textcolor{gray}{$\pm$ 0.11}                        & 0.29 \textcolor{gray}{$\pm$ 0.08}              & 0.51 \textcolor{gray}{$\pm$ 0.12}                \\
Test      & Blue                    & \textbf{0.44 \textcolor{gray}{$\pm$ 0.07}}  & 0.01 \textcolor{gray}{$\pm$ 0.01}                     & 0.09 \textcolor{gray}{$\pm$ 0.06}                     & 0.14 \textcolor{gray}{$\pm$ 0.04}                        & 0.07 \textcolor{gray}{$\pm$ 0.04}                     & 0.32 \textcolor{gray}{$\pm$ 0.05}                     & 0.15 \textcolor{gray}{$\pm$ 0.03}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\ \midrule
Train     & (Blue, Flower, White)   & 0.57 \textcolor{gray}{$\pm$ 0.08}           & 0.43 \textcolor{gray}{$\pm$ 0.07}                     & 0.43 \textcolor{gray}{$\pm$ 0.09}                     & 0.44 \textcolor{gray}{$\pm$ 0.03}                        & \textbf{0.69 \textcolor{gray}{$\pm$ 0.08}}            & 0.68 \textcolor{gray}{$\pm$ 0.07}                     & 0.42 \textcolor{gray}{$\pm$ 0.09}                        & 0.24 \textcolor{gray}{$\pm$ 0.04}              & 0.47 \textcolor{gray}{$\pm$ 0.08}                \\
Test      & Yellow                  & \textbf{0.63 \textcolor{gray}{$\pm$ 0.09}}  & 0.17 \textcolor{gray}{$\pm$ 0.06}                     & 0.07 \textcolor{gray}{$\pm$ 0.02}                     & 0.47 \textcolor{gray}{$\pm$ 0.03}                        & 0.31 \textcolor{gray}{$\pm$ 0.05}                     & 0.17 \textcolor{gray}{$\pm$ 0.07}                     & 0.37 \textcolor{gray}{$\pm$ 0.06}                        & 0.05 \textcolor{gray}{$\pm$ 0.04}              & 0.06 \textcolor{gray}{$\pm$ 0.05}                \\ \midrule
\multicolumn{2}{l}{In-Distribution Avg.}   & 0.61 \textcolor{gray}{$\pm$ 0.08}           & 0.47 \textcolor{gray}{$\pm$ 0.09}                     & 0.45 \textcolor{gray}{$\pm$ 0.11}                     & 0.49 \textcolor{gray}{$\pm$ 0.09}                        & 0.70 \textcolor{gray}{$\pm$ 0.09}                     & \textbf{0.71 \textcolor{gray}{$\pm$ 0.07}}            & 0.44 \textcolor{gray}{$\pm$ 0.10}                        & 0.26 \textcolor{gray}{$\pm$ 0.10}              & 0.48 \textcolor{gray}{$\pm$ 0.10}                \\
\multicolumn{2}{l}{Out-Of-Distribution Avg.}    & \textbf{0.46 \textcolor{gray}{$\pm$ 0.15}}  & 0.10 \textcolor{gray}{$\pm$ 0.08}                     & 0.15 \textcolor{gray}{$\pm$ 0.09}                     & 0.31 \textcolor{gray}{$\pm$ 0.14}                        & 0.21 \textcolor{gray}{$\pm$ 0.11}                     & 0.29 \textcolor{gray}{$\pm$ 0.10}                     & 0.22 \textcolor{gray}{$\pm$ 0.14}                        & 0.06 \textcolor{gray}{$\pm$ 0.06}              & 0.03 \textcolor{gray}{$\pm$ 0.04}               
\\ \bottomrule \\
\end{tabular}
\caption{Success rate on }
\end{table*}


\begin{table*}[]
\centering
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Object} &  \multicolumn{9}{c} {Method}\\
\cmidrule{3-11}
&  & ViT           & BC$_\text{base}$ & BC$_\text{dino}$ & BC & BC-RNN$_\text{base}$ & BC-RNN$_\text{dino}$ & BC-RNN & R3M$_\text{SM}$ & R3M$_\text{flat}$ \\ \midrule
\multirow{4}{*}{Train}    & Yellow Mug          & 0.70 \textcolor{gray}{$\pm$ 0.07}           & 0.53 \textcolor{gray}{$\pm$ 0.03}                     & 0.56 \textcolor{gray}{$\pm$ 0.07}                     & 0.72 \textcolor{gray}{$\pm$ 0.06}                        & 0.78 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.85 \textcolor{gray}{$\pm$ 0.02}}            & 0.69 \textcolor{gray}{$\pm$ 0.11}                        & 0.35 \textcolor{gray}{$\pm$ 0.05}              & 0.65 \textcolor{gray}{$\pm$ 0.05}                \\
                          & Blue Mug            & 0.57 \textcolor{gray}{$\pm$ 0.07}           & 0.39 \textcolor{gray}{$\pm$ 0.08}                     & 0.40 \textcolor{gray}{$\pm$ 0.03}                     & 0.47 \textcolor{gray}{$\pm$ 0.02}                        & 0.58 \textcolor{gray}{$\pm$ 0.07}                     & \textbf{0.65 \textcolor{gray}{$\pm$ 0.02}}            & 0.40 \textcolor{gray}{$\pm$ 0.07}                        & 0.19 \textcolor{gray}{$\pm$ 0.06}              & 0.37 \textcolor{gray}{$\pm$ 0.03}                \\
                          & White Mug           & 0.58 \textcolor{gray}{$\pm$ 0.08}           & 0.50 \textcolor{gray}{$\pm$ 0.04}                     & 0.59 \textcolor{gray}{$\pm$ 0.06}                     & 0.65 \textcolor{gray}{$\pm$ 0.10}                        & 0.63 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.73 \textcolor{gray}{$\pm$ 0.06}}            & 0.55 \textcolor{gray}{$\pm$ 0.07}                        & 0.19 \textcolor{gray}{$\pm$ 0.01}              & 0.35 \textcolor{gray}{$\pm$ 0.04}                \\
                          & Flower Mug          & 0.56 \textcolor{gray}{$\pm$ 0.04}           & 0.49 \textcolor{gray}{$\pm$ 0.04}                     & 0.45 \textcolor{gray}{$\pm$ 0.03}                     & 0.40 \textcolor{gray}{$\pm$ 0.06}                        & 0.65 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.73 \textcolor{gray}{$\pm$ 0.05}}            & 0.46 \textcolor{gray}{$\pm$ 0.11}                        & 0.28 \textcolor{gray}{$\pm$ 0.02}              & 0.40 \textcolor{gray}{$\pm$ 0.06}                \\ \midrule
\multirow{5}{*}{Test}     & Re-textured Mugs    & \textbf{0.51 \textcolor{gray}{$\pm$ 0.04}}  & 0.23 \textcolor{gray}{$\pm$ 0.03}                     & 0.35 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.51 \textcolor{gray}{$\pm$ 0.08}}               & 0.40 \textcolor{gray}{$\pm$ 0.03}                     & 0.50 \textcolor{gray}{$\pm$ 0.01}                     & 0.45 \textcolor{gray}{$\pm$ 0.10}                        & 0.09 \textcolor{gray}{$\pm$ 0.01}              & 0.11 \textcolor{gray}{$\pm$ 0.02}                \\
                          & Teapot              & 0.02 \textcolor{gray}{$\pm$ 0.00}           & 0.02 \textcolor{gray}{$\pm$ 0.00}                     & 0.12 \textcolor{gray}{$\pm$ 0.07}                     & 0.01 \textcolor{gray}{$\pm$ 0.01}                        & 0.11 \textcolor{gray}{$\pm$ 0.07}                     & \textbf{0.19 \textcolor{gray}{$\pm$ 0.03}}            & 0.03 \textcolor{gray}{$\pm$ 0.02}                        & 0.05 \textcolor{gray}{$\pm$ 0.04}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & Pitcher             & \textbf{0.08 \textcolor{gray}{$\pm$ 0.02}}  & 0.05 \textcolor{gray}{$\pm$ 0.06}                     & 0.05 \textcolor{gray}{$\pm$ 0.01}                     & \textbf{0.05 \textcolor{gray}{$\pm$ 0.04}}               & \textbf{0.09 \textcolor{gray}{$\pm$ 0.05}}            & \textbf{0.04 \textcolor{gray}{$\pm$ 0.02}}            & 0.07 \textcolor{gray}{$\pm$ 0.05}                        & 0.03 \textcolor{gray}{$\pm$ 0.01}              & 0.07 \textcolor{gray}{$\pm$ 0.05}                \\
                          & Coffee              & \textbf{0.11 \textcolor{gray}{$\pm$ 0.02}}  & 0.03 \textcolor{gray}{$\pm$ 0.01}                     & 0.04 \textcolor{gray}{$\pm$ 0.02}                     & 0.03 \textcolor{gray}{$\pm$ 0.01}                        & 0.06 \textcolor{gray}{$\pm$ 0.03}                     & 0.07 \textcolor{gray}{$\pm$ 0.02}                     & 0.01 \textcolor{gray}{$\pm$ 0.02}                        & 0.03 \textcolor{gray}{$\pm$ 0.01}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & Kidcup              & \textbf{0.20 \textcolor{gray}{$\pm$ 0.07}}  & 0.04 \textcolor{gray}{$\pm$ 0.03}                     & 0.07 \textcolor{gray}{$\pm$ 0.02}                     & 0.13 \textcolor{gray}{$\pm$ 0.07}                        & 0.06 \textcolor{gray}{$\pm$ 0.03}                     & 0.05 \textcolor{gray}{$\pm$ 0.02}                     & 0.17 \textcolor{gray}{$\pm$ 0.07}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\ \midrule
\multicolumn{2}{l}{In-Distribution Avg.}     & 0.60 \textcolor{gray}{$\pm$ 0.09}           & 0.48 \textcolor{gray}{$\pm$ 0.08}                     & 0.50 \textcolor{gray}{$\pm$ 0.10}                     & 0.56 \textcolor{gray}{$\pm$ 0.15}                        & 0.66 \textcolor{gray}{$\pm$ 0.08}                     & \textbf{0.74 \textcolor{gray}{$\pm$ 0.08}}            & 0.53 \textcolor{gray}{$\pm$ 0.14}                        & 0.25 \textcolor{gray}{$\pm$ 0.08}              & 0.44 \textcolor{gray}{$\pm$ 0.13}                \\
\multicolumn{2}{l}{Out-Of-Distribution Avg.} & \textbf{0.18 \textcolor{gray}{$\pm$ 0.18}}  & 0.07 \textcolor{gray}{$\pm$ 0.09}                     & 0.13 \textcolor{gray}{$\pm$ 0.12}                     & 0.15 \textcolor{gray}{$\pm$ 0.20}                        & 0.14 \textcolor{gray}{$\pm$ 0.14}                     & 0.17 \textcolor{gray}{$\pm$ 0.17}                     & 0.15 \textcolor{gray}{$\pm$ 0.17}                        & 0.04 \textcolor{gray}{$\pm$ 0.04}              & 0.04 \textcolor{gray}{$\pm$ 0.05} \\
\bottomrule \\
\end{tabular}
\caption{Experiment2}
\end{table*}



\begin{table*}[]
\centering
\begin{tabular}{@{}llccccccccc@{}}
\toprule
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Object} &  \multicolumn{9}{c} {Method}\\
\cmidrule{3-11}
           &  & ViT           & BC$_\text{base}$ & BC$_\text{dino}$ & BC & BC-RNN$_\text{base}$ & BC-RNN$_\text{dino}$ & BC-RNN & R3M$_\text{SM}$ & R3M$_\text{flat}$ \\ \midrule
\multirow{3}{*}{Train}    & Yellow Mug          & 0.52 \textcolor{gray}{$\pm$ 0.03}           & 0.37 \textcolor{gray}{$\pm$ 0.04}                     & 0.38 \textcolor{gray}{$\pm$ 0.06}                     & 0.43 \textcolor{gray}{$\pm$ 0.07}                        & \textbf{0.71 \textcolor{gray}{$\pm$ 0.08}}            & 0.69 \textcolor{gray}{$\pm$ 0.06}                     & 0.31 \textcolor{gray}{$\pm$ 0.12}                        & 0.23 \textcolor{gray}{$\pm$ 0.03}              & 0.47 \textcolor{gray}{$\pm$ 0.01}                \\
                          & Pan                 & 0.83 \textcolor{gray}{$\pm$ 0.02}           & 0.71 \textcolor{gray}{$\pm$ 0.06}                     & 0.69 \textcolor{gray}{$\pm$ 0.07}                     & 0.69 \textcolor{gray}{$\pm$ 0.03}                        & 0.89 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.89 \textcolor{gray}{$\pm$ 0.03}}            & 0.71 \textcolor{gray}{$\pm$ 0.05}                        & 0.40 \textcolor{gray}{$\pm$ 0.11}              & 0.69 \textcolor{gray}{$\pm$ 0.05}                \\
                          & Screwdriver         & \textbf{0.91 \textcolor{gray}{$\pm$ 0.02}}  & 0.67 \textcolor{gray}{$\pm$ 0.02}                     & 0.73 \textcolor{gray}{$\pm$ 0.05}                     & 0.87 \textcolor{gray}{$\pm$ 0.03}                        & 0.89 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.91 \textcolor{gray}{$\pm$ 0.05}}            & 0.76 \textcolor{gray}{$\pm$ 0.07}                        & 0.44 \textcolor{gray}{$\pm$ 0.11}              & 0.79 \textcolor{gray}{$\pm$ 0.05}                \\ \midrule
\multirow{21}{*}{Test}    & MugBlue             & \textbf{0.47 \textcolor{gray}{$\pm$ 0.01}}  & 0.06 \textcolor{gray}{$\pm$ 0.00}                     & 0.10 \textcolor{gray}{$\pm$ 0.03}                     & 0.20 \textcolor{gray}{$\pm$ 0.04}                        & 0.11 \textcolor{gray}{$\pm$ 0.02}                     & 0.03 \textcolor{gray}{$\pm$ 0.03}                     & 0.08 \textcolor{gray}{$\pm$ 0.06}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & MugWhite            & 0.25 \textcolor{gray}{$\pm$ 0.04}           & 0.05 \textcolor{gray}{$\pm$ 0.02}                     & 0.14 \textcolor{gray}{$\pm$ 0.03}                     & \textbf{0.41 \textcolor{gray}{$\pm$ 0.05}}               & 0.09 \textcolor{gray}{$\pm$ 0.03}                     & 0.15 \textcolor{gray}{$\pm$ 0.05}                     & 0.19 \textcolor{gray}{$\pm$ 0.06}                        & 0.05 \textcolor{gray}{$\pm$ 0.01}              & 0.02 \textcolor{gray}{$\pm$ 0.02}                \\
                          & MugFlower           & 0.30 \textcolor{gray}{$\pm$ 0.06}           & 0.05 \textcolor{gray}{$\pm$ 0.02}                     & 0.09 \textcolor{gray}{$\pm$ 0.02}                     & \textbf{0.32 \textcolor{gray}{$\pm$ 0.11}}               & 0.14 \textcolor{gray}{$\pm$ 0.02}                     & 0.21 \textcolor{gray}{$\pm$ 0.02}                     & 0.19 \textcolor{gray}{$\pm$ 0.04}                        & 0.07 \textcolor{gray}{$\pm$ 0.02}              & 0.04 \textcolor{gray}{$\pm$ 0.03}                \\
                          & TeapotWhite         & 0.14 \textcolor{gray}{$\pm$ 0.06}           & 0.04 \textcolor{gray}{$\pm$ 0.03}                     & 0.04 \textcolor{gray}{$\pm$ 0.02}                     & 0.05 \textcolor{gray}{$\pm$ 0.01}                        & 0.03 \textcolor{gray}{$\pm$ 0.01}                     & 0.15 \textcolor{gray}{$\pm$ 0.03}                     & 0.00 \textcolor{gray}{$\pm$ 0.00}                        & 0.01 \textcolor{gray}{$\pm$ 0.01}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & PitcherWhite        & 0.08 \textcolor{gray}{$\pm$ 0.04}           & 0.03 \textcolor{gray}{$\pm$ 0.01}                     & 0.01 \textcolor{gray}{$\pm$ 0.01}                     & \textbf{0.11 \textcolor{gray}{$\pm$ 0.10}}               & 0.05 \textcolor{gray}{$\pm$ 0.02}                     & 0.04 \textcolor{gray}{$\pm$ 0.04}                     & 0.07 \textcolor{gray}{$\pm$ 0.04}                        & 0.06 \textcolor{gray}{$\pm$ 0.03}              & 0.07 \textcolor{gray}{$\pm$ 0.04}                \\
                          & Coffee              & \textbf{0.09 \textcolor{gray}{$\pm$ 0.03}}  & 0.03 \textcolor{gray}{$\pm$ 0.02}                     & 0.08 \textcolor{gray}{$\pm$ 0.03}                     & 0.08 \textcolor{gray}{$\pm$ 0.03}                        & 0.06 \textcolor{gray}{$\pm$ 0.03}                     & 0.08 \textcolor{gray}{$\pm$ 0.05}                     & 0.05 \textcolor{gray}{$\pm$ 0.02}                        & 0.05 \textcolor{gray}{$\pm$ 0.04}              & 0.03 \textcolor{gray}{$\pm$ 0.02}                \\
                          & Kidcup              & \textbf{0.10 \textcolor{gray}{$\pm$ 0.03}}  & 0.04 \textcolor{gray}{$\pm$ 0.06}                     & 0.02 \textcolor{gray}{$\pm$ 0.02}                     & 0.06 \textcolor{gray}{$\pm$ 0.02}                        & 0.01 \textcolor{gray}{$\pm$ 0.01}                     & 0.05 \textcolor{gray}{$\pm$ 0.07}                     & 0.03 \textcolor{gray}{$\pm$ 0.02}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          \cmidrule{3-11}
                          & Hammer              & 0.51 \textcolor{gray}{$\pm$ 0.04}           & 0.43 \textcolor{gray}{$\pm$ 0.06}                     & 0.49 \textcolor{gray}{$\pm$ 0.11}                     & 0.59 \textcolor{gray}{$\pm$ 0.05}                        & 0.63 \textcolor{gray}{$\pm$ 0.09}                     & \textbf{0.67 \textcolor{gray}{$\pm$ 0.04}}            & 0.49 \textcolor{gray}{$\pm$ 0.05}                        & 0.19 \textcolor{gray}{$\pm$ 0.06}              & 0.19 \textcolor{gray}{$\pm$ 0.06}                \\
                          & Spatula             & 0.59 \textcolor{gray}{$\pm$ 0.09}           & 0.15 \textcolor{gray}{$\pm$ 0.04}                     & 0.35 \textcolor{gray}{$\pm$ 0.01}                     & \textbf{0.73 \textcolor{gray}{$\pm$ 0.03}}               & 0.33 \textcolor{gray}{$\pm$ 0.04}                     & 0.43 \textcolor{gray}{$\pm$ 0.11}                     & 0.62 \textcolor{gray}{$\pm$ 0.06}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & MagGlass            & \textbf{0.29 \textcolor{gray}{$\pm$ 0.02}}  & 0.05 \textcolor{gray}{$\pm$ 0.01}                     & 0.01 \textcolor{gray}{$\pm$ 0.01}                     & 0.14 \textcolor{gray}{$\pm$ 0.06}                        & 0.11 \textcolor{gray}{$\pm$ 0.05}                     & 0.03 \textcolor{gray}{$\pm$ 0.01}                     & 0.02 \textcolor{gray}{$\pm$ 0.03}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & HairStraightener    & 0.50 \textcolor{gray}{$\pm$ 0.04}           & 0.29 \textcolor{gray}{$\pm$ 0.08}                     & 0.15 \textcolor{gray}{$\pm$ 0.01}                     & \textbf{0.55 \textcolor{gray}{$\pm$ 0.09}}               & 0.33 \textcolor{gray}{$\pm$ 0.07}                     & 0.18 \textcolor{gray}{$\pm$ 0.07}                     & 0.37 \textcolor{gray}{$\pm$ 0.05}                        & 0.09 \textcolor{gray}{$\pm$ 0.05}              & 0.08 \textcolor{gray}{$\pm$ 0.03}                \\
                          & Spoonrest           & 0.51 \textcolor{gray}{$\pm$ 0.11}           & 0.27 \textcolor{gray}{$\pm$ 0.03}                     & 0.38 \textcolor{gray}{$\pm$ 0.06}                     & 0.38 \textcolor{gray}{$\pm$ 0.04}                        & 0.43 \textcolor{gray}{$\pm$ 0.05}                     & \textbf{0.57 \textcolor{gray}{$\pm$ 0.05}}            & 0.11 \textcolor{gray}{$\pm$ 0.06}                        & 0.12 \textcolor{gray}{$\pm$ 0.03}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & DustPan             & \textbf{0.32 \textcolor{gray}{$\pm$ 0.06}}  & 0.09 \textcolor{gray}{$\pm$ 0.05}                     & 0.25 \textcolor{gray}{$\pm$ 0.02}                     & 0.19 \textcolor{gray}{$\pm$ 0.08}                        & 0.23 \textcolor{gray}{$\pm$ 0.03}                     & 0.29 \textcolor{gray}{$\pm$ 0.02}                     & 0.08 \textcolor{gray}{$\pm$ 0.03}                        & 0.03 \textcolor{gray}{$\pm$ 0.01}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          \cmidrule{3-11}
                          & Basket              & 0.16 \textcolor{gray}{$\pm$ 0.03}           & 0.12 \textcolor{gray}{$\pm$ 0.07}                     & 0.13 \textcolor{gray}{$\pm$ 0.08}                     & 0.16 \textcolor{gray}{$\pm$ 0.06}                        & \textbf{0.19 \textcolor{gray}{$\pm$ 0.06}}            & 0.04 \textcolor{gray}{$\pm$ 0.06}                     & 0.06 \textcolor{gray}{$\pm$ 0.08}                        & 0.01 \textcolor{gray}{$\pm$ 0.02}              & 0.01 \textcolor{gray}{$\pm$ 0.01}                \\
                          & Bell                & \textbf{0.30 \textcolor{gray}{$\pm$ 0.10}}  & 0.07 \textcolor{gray}{$\pm$ 0.01}                     & 0.15 \textcolor{gray}{$\pm$ 0.05}                     & 0.22 \textcolor{gray}{$\pm$ 0.13}                        & 0.22 \textcolor{gray}{$\pm$ 0.09}                     & 0.13 \textcolor{gray}{$\pm$ 0.09}                     & 0.29 \textcolor{gray}{$\pm$ 0.15}                        & 0.04 \textcolor{gray}{$\pm$ 0.03}              & 0.01 \textcolor{gray}{$\pm$ 0.01}                \\
                          & CClamp              & 0.05 \textcolor{gray}{$\pm$ 0.04}           & 0.03 \textcolor{gray}{$\pm$ 0.04}                     & 0.10 \textcolor{gray}{$\pm$ 0.06}                     & 0.21 \textcolor{gray}{$\pm$ 0.02}                        & \textbf{0.21 \textcolor{gray}{$\pm$ 0.09}}            & 0.14 \textcolor{gray}{$\pm$ 0.04}                     & 0.07 \textcolor{gray}{$\pm$ 0.05}                        & 0.08 \textcolor{gray}{$\pm$ 0.04}              & 0.03 \textcolor{gray}{$\pm$ 0.01}                \\
                          & Honeydip            & 0.03 \textcolor{gray}{$\pm$ 0.02}           & 0.17 \textcolor{gray}{$\pm$ 0.06}                     & 0.17 \textcolor{gray}{$\pm$ 0.10}                     & 0.03 \textcolor{gray}{$\pm$ 0.02}                        & 0.07 \textcolor{gray}{$\pm$ 0.05}                     & \textbf{0.27 \textcolor{gray}{$\pm$ 0.16}}            & 0.04 \textcolor{gray}{$\pm$ 0.06}                        & 0.03 \textcolor{gray}{$\pm$ 0.02}              & 0.01 \textcolor{gray}{$\pm$ 0.01}                \\
                          & Shoe1               & \textbf{0.30 \textcolor{gray}{$\pm$ 0.03}}  & 0.20 \textcolor{gray}{$\pm$ 0.03}                     & 0.25 \textcolor{gray}{$\pm$ 0.10}                     & 0.24 \textcolor{gray}{$\pm$ 0.06}                        & 0.21 \textcolor{gray}{$\pm$ 0.07}                     & 0.27 \textcolor{gray}{$\pm$ 0.07}                     & 0.10 \textcolor{gray}{$\pm$ 0.05}                        & 0.06 \textcolor{gray}{$\pm$ 0.07}              & 0.01 \textcolor{gray}{$\pm$ 0.01}                \\
                          & Shoe2               & 0.28 \textcolor{gray}{$\pm$ 0.06}           & 0.13 \textcolor{gray}{$\pm$ 0.04}                     & 0.22 \textcolor{gray}{$\pm$ 0.02}                     & 0.17 \textcolor{gray}{$\pm$ 0.02}                        & 0.26 \textcolor{gray}{$\pm$ 0.06}                     & \textbf{0.42 \textcolor{gray}{$\pm$ 0.07}}            & 0.10 \textcolor{gray}{$\pm$ 0.03}                        & 0.12 \textcolor{gray}{$\pm$ 0.05}              & 0.00 \textcolor{gray}{$\pm$ 0.00}                \\
                          & Rattle              & \textbf{0.45 \textcolor{gray}{$\pm$ 0.14}}  & 0.14 \textcolor{gray}{$\pm$ 0.08}                     & 0.13 \textcolor{gray}{$\pm$ 0.02}                     & 0.24 \textcolor{gray}{$\pm$ 0.08}                        & 0.16 \textcolor{gray}{$\pm$ 0.05}                     & 0.13 \textcolor{gray}{$\pm$ 0.07}                     & 0.13 \textcolor{gray}{$\pm$ 0.10}                        & 0.10 \textcolor{gray}{$\pm$ 0.06}              & 0.08 \textcolor{gray}{$\pm$ 0.03}                \\
                          & LionToy             & \textbf{0.21 \textcolor{gray}{$\pm$ 0.05}}  & 0.19 \textcolor{gray}{$\pm$ 0.08}                     & 0.03 \textcolor{gray}{$\pm$ 0.02}                     & 0.16 \textcolor{gray}{$\pm$ 0.04}                        & 0.09 \textcolor{gray}{$\pm$ 0.01}                     & 0.04 \textcolor{gray}{$\pm$ 0.04}                     & 0.04 \textcolor{gray}{$\pm$ 0.02}                        & 0.00 \textcolor{gray}{$\pm$ 0.00}              & 0.01 \textcolor{gray}{$\pm$ 0.01}                \\ \midrule  
\multicolumn{2}{l}{In-Distribution Avg.}     & 0.76 \textcolor{gray}{$\pm$ 0.17}           & 0.58 \textcolor{gray}{$\pm$ 0.16}                     & 0.60 \textcolor{gray}{$\pm$ 0.17}                     & 0.67 \textcolor{gray}{$\pm$ 0.19}                        & \textbf{0.83 \textcolor{gray}{$\pm$ 0.10}}            & \textbf{0.83 \textcolor{gray}{$\pm$ 0.11}}            & 0.59 \textcolor{gray}{$\pm$ 0.22}                        & 0.36 \textcolor{gray}{$\pm$ 0.13}              & 0.65 \textcolor{gray}{$\pm$ 0.14}                \\
\multicolumn{2}{l}{Out-Of-Distribution Avg.} & \textbf{0.28 \textcolor{gray}{$\pm$ 0.18}}  & 0.12 \textcolor{gray}{$\pm$ 0.11}                     & 0.16 \textcolor{gray}{$\pm$ 0.14}                     & 0.25 \textcolor{gray}{$\pm$ 0.19}                        & 0.19 \textcolor{gray}{$\pm$ 0.15}                     & 0.21 \textcolor{gray}{$\pm$ 0.19}                     & 0.15 \textcolor{gray}{$\pm$ 0.17}                        & 0.05 \textcolor{gray}{$\pm$ 0.06}              & 0.03 \textcolor{gray}{$\pm$ 0.05} \\
\bottomrule \\
\end{tabular}
\caption{Experiment3}
\end{table*}
